Generative Adversarial Neural Operators

We propose the generative adversarial neural operator (GANO), a generative model paradigm for learning probabilities on infinite-dimensional function spaces. The natural sciences and engineering are known to have many types of data that are sampled from infinite-dimensional function spaces, where classical finite-dimensional deep generative adversarial networks (GANs) may not be directly applicable. GANO generalizes the GAN framework and allows for the sampling of functions by learning push-forward operator maps in infinite-dimensional spaces. GANO consists of two main components, a generator neural operator and a discriminator neural functional. The inputs to the generator are samples of functions from a user-specified probability measure, e.g., Gaussian random field (GRF), and the generator outputs are synthetic data functions. The input to the discriminator is either a real or synthetic data function. In this work, we instantiate GANO using the Wasserstein criterion and show how the Wasserstein loss can be computed in infinite-dimensional spaces. We empirically study GANO in controlled cases where both input and output functions are samples from GRFs and compare its performance to the finite-dimensional counterpart GAN. We empirically study the efficacy of GANO on real-world function data of volcanic activities and show its superior performance over GAN.

==> Sections/3-Preliminaries.tex <==
\section{Preliminaries}
Let $\A$ and $\U$ denote Polish function spaces, such that for any $a\in\A$, $a:D_\A\rightarrow\Real^{d_\A}$ and for $u\in\U$, $u:D_\U\rightarrow\Real^{d_\U}$.  
Let $\bG$ denote a space of operators and for any operator $\G\in\bG$, we have $\G:\A\rightarrow\U$, an operator map from $\A$ to $\U$. Let $\bL$ denote a space of functionals and for any functional $d\in\bL$, we have $d:\U\rightarrow\Real$, a functional map from $\U$ to $\Real$.

Let $(\A,\sigma(\A),P_\A)$ denote the probability space induced by a Gaussian random field on function spaces $\A$, and $(\U,\sigma(\U),P_\U)$ denote a probability space on the function spaces $\U$. 

For a given function space $\U$, let $\U^*$ denote the dual space of $U$.
When $\U$ is also a Banach space, and $\G$ is Fr\'echet differentiable, we define $\partial\G$ as the Fr\'echet derivative of $\G$. 

==> Sections/4.1-architecture_old.tex <==
\subsection{\GANO Architecture}\label{subsec:arch}

Neural Operators are deep learning models that are the building blocks of the generator and discriminator architectures in \GANO to learn maps between function spaces, and the space of reals. In this work, we utilize the \UNO architecture \citep{UNO} for its efficiency, stability, and robustness to the choice of hyper parameters. We implement the generator operator $\G$ using an eight-layered neural operator model. The inputs to the $\G$ model are samples generated from a \GRF defined on the 2D domain of $\D = [0,1]^2$. The output of $\G$, and $u$'s are sample functions that are defined on a 2D domain. In the following, we describe the detail of the generator. For any function $a$ drawn from the input \GRF, the generator first applies a pointwise operator $\P$, parameterized with an one layered neural network $P$, to compute $\nu_0$, i.e., $\nu_0(x) = P(a(x))~\forall x\in\D$. Let $\D_0$ denote the domain functions for which $\nu_0$ is defined in. Given the application of $\P$, we have $\D_0=\D$. This point-wise operator layer is followed by $L$ integral layers. For any layer $i$, we have,

\[
\nu_{i+1}(y) = \int_{\D_i}k_i(x,y)\nu_i(x)d\mu_i(y),\quad\forall y\in\D_{i+1}
\]
where $k_i$ is the kernel function and the $d\mu_i$ is the measure in the $i$'th layer. We deploy convolution theorem to compute this integral as proposed in~\citet{li2020fourier}. After $L$ integral layers and computing $\nu_L$ defined on the domain $\D_L=\D$, we apply the final pointwise operator $\Q$, parameterized with a two layered neural network $Q$. It is such that for any $x\in\D$, we have $u(x)=Q(\nu_L(x))$. This constitutes the generator model $\G$ which outputs a function $u$ given a sample function $a$, i.e., $u=\G(a)$. 



The discriminator is a neural functional that consists of an eight-layer neural operator followed by an integral functional that maps the output function of the neural operator to a number in $\Real$. In other words, we feed an input function $u\in\U$ to the neural operator part of the discriminator to compute the intermediate function $h$ and the output of the discriminator $r\in \Real$ is computed as, 

\begin{equation} \label{eq:d_fno}
r:= d(u) = \int k_d(x)h(x)dx
\end{equation}

where the function $k_d$ is parameterized as a 3-layered fully connected neural network. Note that $h$ is the output of the inner neural operator with $u$ as an input, therefore, $h$ directly depends on $u$. The function $k_d$ constitutes the integral functional $\int k_d(x)$ which acts point-wise on its input function. This linear integral functional as the last layer is the direct generalization of the last layer of discriminators in \GAN models to map a function to a number. In many \GAN models, the last layer maps a high dimensional vector to a number. This step is accomplished by a vector-vector inner product. Such a product, in continuum, resembles function-function inner product, i.e., the act of linear integral functional. This also directly follows the Riesz representation theorem~\cite{walter1974real} stating that, under suitable construction, a linear functional (map from infinite dimension to the space of reals) can be written as a linear integral functional. Fig.~\ref{fig:cartoon_gano} demonstrate the architecture of the generator $\G$ and the discriminator $d$.




We represent the input function on a grid of $m_1 \times m_2$. It allows us to use auto-grad to compute the gradient penalty for the Wasserstein loss. Following the function space definitions, the gradient penalty using the auto-grad call of $\nabla d(u)$ is implemented as $\E_{\Prob'_\A}(||\nabla d(u)||-1/\sqrt{m_1m_2})^2$ which is different than the finite-dimensional view in \GAN. The choice of $\sqrt{m_1m_2}$ arises from the fact that we use the Lebesgue measure on $\D_\U$ to define the space $\U$. This ratio resembles that the basis functions deployed to represent the function $u$ on the grid of $m_1\times m_2$ need to be chosen and scaled according to $m_1m_2$ due to the fact that the basis functions are functions with unit norms in the metric space $\U$ with $L^2$ as the metric. It is important to note that since we compute the gradient with the consideration of the underlying metric space, the gradient computation using auto-grad is resolution invariant. Ergo, any resolution of choice can be used to train \GANO models, fulfilling the premise of learning in infinite-dimensional spaces. Note that, for irregular grids where measures other than the deployed Lebesgue measures are used, this calculation should be adapted properly. 




==> Sections/Acknowledgements.tex <==
\subsection*{Acknowledgements}
The authors thank Yuan-Kai Liu for his assistance in preparing the InSAR dataset. The authors would like to thank Zongyi Li and Hongkai Zheng for their valuable inputs. Anima Anandkumar and Zachary E. Ross are supported in part by Carver Mead New Adventures Fund.

==> macros.tex <==
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand{\DS}{D_S}
\newcommand{\weight}{w}
\DeclareMathOperator{\Tr}{Tr}

\newcommand{\barkernel}{\bar\kappa}

\newcommand{\Eone}{\textbf{E1}}
\newcommand{\Etwo}{\textbf{E2}}
\newcommand{\Ethree}{\textbf{E3}}
\newcommand{\Efour}{\textbf{E4}}

\newcommand{\kernel}{\kappa}
\newcommand{\FuncClass}{\mathbb{F}}
\newcommand{\GuncClass}{\mathbb{G}}
\newcommand{\Rade}{\mathcal{R}}
\newcommand{\Order}{\mathcal{O}}
\newcommand{\loss}{{L}}
\newcommand{\impW}{\omega}
\newcommand{\impWv}{\impW_\varepsilon}
\newcommand{\imptheta}{\theta}
\newcommand{\impthetaV}{\theta}
\newcommand{\DT}{D_T}
\newcommand{\impV}{\omega}
\newcommand{\VecOne}{\textbf{1}}
\newcommand{\FunOne}{\mathbbm{1}}
\newcommand{\Dpg}{\Delta_{p_g}}
\newcommand{\Dqg}{\Delta_{q_g}}
\newcommand{\DTg}{\Delta_{T_g}}
\newcommand{\Dpu}{\Delta_{p_u}}
\newcommand{\Dqu}{\Delta_{q_u}}
\newcommand{\DTu}{\Delta_{\T_u}}
\newcommand{\measures}{\mathcal{P}}
\newcommand{\hmax}{h_{\max}}
\newcommand{\umax}{u_{\max}}
\newcommand{\impthetamax}{\imptheta_{\max}}
\newcommand{\G}{\mathcal{G}}




\newcommand{\Comp}{\mathbb{C}}
\newcommand{\HS}{\mathcal{HS}}
\newcommand{\Hilbert}{\mathcal{H}}
\newcommand{\ttt}{\tilde{\Theta}}
\newcommand{\dinf}{d_{\infty}}
\newcommand{\tth}{\hat{\Theta}}
\newcommand{\tts}{\Theta_*}
\newcommand{\ta}{\tilde{A}}
\newcommand{\tb}{\tilde{B}}
\newcommand{\tc}{\tilde{C}}
\newcommand{\tp}{\tilde{P}}
\newcommand{\tl}{\tilde{L}}
\newcommand{\tk}{\tilde{K}}
\newcommand{\Texp}{T_{exp}}
\newcommand{\Tw}{T_{w}}
\newcommand{\Tres}{T_{reset}}
\newcommand{\Alg}{\textsc{\small{LqgOpt}}\xspace}
\newcommand{\ERM}{\textsc{\small{ERM}}\xspace}
\newcommand{\Sys}{\textsc{\small{SysId}}\xspace}

\newcommand{\reg}{\textsc{\small{REGRET}}\xspace}
\newcommand{\OO}{\mathcal{O}}
\newcommand{\RL}{\textsc{\small{RL}}\xspace}
\newcommand{\LQR}{\textsc{\small{LQR}}\xspace}
\newcommand{\LQG}{\textsc{\small{LQG}}\xspace}
\newcommand{\OFU}{\textsc{\small{OFU}}\xspace}

\newcommand{\alg}{\textsc{\small{LqgOpt}}\xspace}
% \newcommand{\LQG}{\textsc{\small{LQG}}\xspace}
% \newcommand{\OFU}{\textsc{\small{OFU}}\xspace}
\newcommand{\POMDP}{\textsc{\small{POMDP}}\xspace}
\newcommand{\MDP}{\textsc{\small{MDP}}\xspace}
\newcommand{\trpo}{\textsc{\small{TRPO}}\xspace}
\newcommand{\ppo}{\textsc{\small{PPO}}\xspace}
\newcommand{\PPO}{\textsc{\small{PPO}}\xspace}
\newcommand*{\Scale}[2][4]{\scalebox{#1}{$#2$}}
\newcommand{\vecy}{\vec y}
\newcommand{\history}{\mathfrak{H}}
\newcommand{\trans}{T}
\newcommand{\obs}{O}
% \newcommand{\Texp}{T_{exp}}
\newcommand{\Dexp}{\mathcal{D}_{exp}}
\newcommand{\Gcl}{\mathcal{G}^{cl}}
\newcommand{\Gol}{\mathcal{G}^{ol}}


\newcommand{\policy}{\Pi}
\newcommand{\vpi}{{\pi}}
\newcommand{\vobs}{\vec{o}}
\newcommand{\stait}{\omega}
\newcommand{\rxa}{\Gamma}
\newcommand{\rya}{\Upsilon}
\newcommand{\U}{\mathcal{U}}
\newcommand{\Est}{M_1}
\newcommand{\End}{M_2}
\newcommand{\Erd}{M_3}
\newcommand{\decompos}{\gamma}
\newcommand{\pertM}{\Delta M_3}
\newcommand{\pertMM}{\Delta \tilde{M_3}}
\newcommand{\samplenum}{m_s}
\newcommand{\reward}{\Psi}
\newcommand{\tuple}{\mathcal{M}}
\newcommand{\bellman}{\mathcal{E}}
\newcommand{\whole}{\tilde{\mathcal{M}}}
\newcommand{\approxim}{\breve{\mathcal{M}}}
\newcommand{\subst}{{\breve{\eta}}_{\vpi^*}}
\newcommand{\effect}{v}
\newcommand{\belief}{b}
\newcommand{\cost}{c}
\newcommand{\val}{J}
\newcommand{\Qfunc}{Q}

\newcommand{\block}{\Xi}
\newcommand{\vect}{Vec}
\newcommand{\rprob}{z}
\newcommand{\past}{n}
\newcommand{\OPRE}{\textsc{\small{OPRE}}\xspace}
\newcommand{\OPREIS}{\textsc{\small{OPRE-IS}}\xspace}
\newcommand{\BF}{\textsc{BF}\xspace}
% \newcommand{\IS}{\textsc{\small{IS}}\xspace}
\newcommand{\tslive}{\textsc{\small{TS-LIVE}}\xspace}
\newcommand{\olive}{\textsc{\small{OLIVE}}\xspace}
\newcommand{\cdp}{\textsc{{CDP}}\xspace}
\newcommand{\CDF}{\textsc{{CDF}}\xspace}
\newcommand{\cdps}{\textsc{{CDPs}}\xspace}
\newcommand{\ts}{\textsc{TS}\xspace}
\newcommand{\IS}{\textsc{IS}\xspace}
\newcommand{\ISClip}{\textsc{IS-Clip}\xspace}
\newcommand{\DR}{\textsc{DR}\xspace}
\newcommand{\ofu}{\textsc{OFU}\xspace}
\newcommand{\mdp}{\textsc{\small{MDP}}\xspace}
\newcommand{\pomdp}{\textsc{\small{POMDP}}\xspace}
\newcommand{\Azuma}{\mathcal{J}}
\newcommand{\Dr}{D_{\text{ratio}}}
\newcommand{\Ke}{\mathcal{K}_\epsilon}
\newcommand{\Le}{L_\epsilon}
\newcommand{\w}{W}
\newcommand{\VV}{B}
\newcommand{\vv}{b}
\newcommand{\HH}{S}
\newcommand{\hhh}{s}
\newcommand{\deltaO}{d_O}

\newcommand*{\defeq}{\mathrel{\vcenter{\baselineskip0.5ex \lineskiplimit0pt
                     \hbox{\scriptsize.}\hbox{\scriptsize.}}}%
                     =}

% Misc symbols
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Borel}{\mathbb{B}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\calP}{\mathcal P}
\newcommand{\F}{\mathcal F}
\newcommand{\Z}{\mathcal Z}
\newcommand{\A}{\mathcal A}
\newcommand{\P}{\mathcal P}
\newcommand{\B}{\mathcal B}
\newcommand{\X}{\mathcal X}
\newcommand{\W}{\mathcal W}
\newcommand{\T}{\mathcal T}
\newcommand{\KL}{\mathcal D_{KL}}
\newcommand{\wKL}{\wh{\mathcal{D}}_{KL}}
\newcommand{\D}{\mathcal D}
\newcommand{\Gr}{\nabla_{\theta}}
\newcommand{\Greta}{\nabla \eta}
\newcommand{\Grrho}{\nabla \rho}
\newcommand{\Grphi}{\nabla_\phi}
\newcommand{\adv}{A}
\newcommand{\TN}{N}
\newcommand{\hh}{\hat h}
\newcommand{\hL}{\hat L}
\renewcommand{\L}{\mathcal L}
\newcommand{\Hyp}{\mathcal H}
\newcommand{\Y}{\mathcal Y}
\newcommand{\V}{\mathcal V}
\newcommand{\M}{\mathcal M}
\renewcommand{\S}{\mathcal S}
\newcommand{\C}{\mathcal C}
\newcommand{\K}{\mathcal K}
\newcommand{\E}{\mathbb E}
\newcommand{\calE}{\mathcal E}
\newcommand{\cov}{\textnormal{Cov}}
%\newcommand{\V}{\mathbb V}
\newcommand{\Prob}{\mathbb P}
\newcommand{\Ind}{\mathbbm{1}}
\newcommand{\Qrob}{\mathbb Q}
\newcommand{\I}{\mathbbm 1}
\newcommand{\N}{\mathcal N}
\newcommand{\balpha}{\boldsymbol \alpha}
\newcommand{\bmu}{\boldsymbol \mu}
\newcommand{\bSigma}{\boldsymbol \Sigma}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\MV}{\textnormal{MV}}
\newcommand{\hMV}{\widehat{\textnormal{MV}}}
\newcommand{\barmu}{\bar\mu}
\newcommand{\hmu}{\hat\mu}
\newcommand{\tmu}{\tilde\mu}
\newcommand{\barvar}{\bar\sigma^2}
%\newcommand{\hvar}{\hat\sigma^2}
\newcommand{\tvar}{\tilde\sigma^2}
\newcommand{\R}{\mathfrak{R}}
\newcommand{\hR}{\widehat{\mathcal{R}}}
\newcommand{\tR}{\widetilde{\mathcal R}}
\newcommand{\Cb}{{\mtx{C}}}
%\newcommand{\var}{\sigma^2}
\newcommand{\invdelta}{1/\delta}
\newcommand{\boldR}{\mathbb R}
\newcommand{\eps}{\varepsilon}
\newcommand{\mvlcb}{\textnormal{\texttt{MV-LCB }}}
\newcommand{\clip}{\textnormal{\texttt{Clip}}}
\newcommand{\epsMonoton}{\epsilon_{\M}}
\newcommand{\ucb}{\textnormal{\textsl{UCB }}}
\newcommand{\GANO}{\textnormal{\textsl{GANO}}}
\newcommand{\GAN}{\textnormal{\textsl{GAN}}}
\newcommand{\ucbv}{\textnormal{\textsl{UCB-V }}}
\newcommand{\mvlcbt}{\textnormal{\texttt{MV-LCB(t) }}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hi}{\hat{i}}
\newcommand{\btheta}{\bar{\theta}}
\newcommand{\tTheta}{\widetilde{\Theta}}



\newcommand{\CVaR}{\textnormal{CVaR}}
\newcommand{\VaR}{\textnormal{C}}
\newcommand{\hcvar}{\widehat{\textnormal{C}}}
\newcommand{\var}{\textnormal{V}}
\newcommand{\varXA}{\sigma^2}
\newcommand{\EXA}{G}
\newcommand{\Var}{\mathbb{V}}
\newcommand{\Cov}{\mathbb{C}}
\newcommand{\hvar}{\widehat{\textnormal{V}}}
\newcommand{\Pinit}{P_\varnothing}



\newcommand{\avg}[2]{\frac{1}{#2} \sum_{#1=1}^{#2}}
\newcommand{\hDelta}{\widehat{\Delta}}
\newcommand{\hGamma}{\widehat{\Gamma}}

\newcommand{\wt}{\widetilde}
\newcommand{\wh}{\widehat}
\newcommand{\wb}{\overline}
 \newcommand{\mbb}{\mathbbm}
\newcommand{\cvara}{\text{CVaR}_\alpha}

% Propositions
%
%\newtheoremstyle{dotless}{}{}{\itshape}{}{\bfseries}{}{ }{}
%\theoremstyle{dotless}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{proof}{Proof}[section]
\newtheorem{proof*}{Proof}[section]
% \newtheorem{assumption}{Assumption}[section]
% \newtheorem{theorem*}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

